NTIRE 2025 Challenge on Cross-Domain Few-Shot Object Detection: Methods and Results

Cross-Domain Few-Shot Object Detection (CD-FSOD) poses significant challenges to existing object detection and few-shot detection models when applied across domains. In conjunction with NTIRE 2025, we organized the 1st CD-FSOD Challenge, aiming to advance the performance of current object detectors on entirely novel target domains with only limited labeled data. The challenge attracted 152 registered participants, received submissions from 42 teams, and concluded with 13 teams making valid final submissions. Participants approached the task from diverse perspectives, proposing novel models that achieved new state-of-the-art (SOTA) results under both open-source and closed-source settings. In this report, we present an overview of the 1st NTIRE 2025 CD-FSOD Challenge, highlighting the proposed solutions and summarizing the results submitted by the participants.

==> teams/affiliation.tex <==
\subsection*{Your team name}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team00_Example/affiliation.tex <==
\subsection*{Example}
\noindent\textit{\textbf{Title: }}Cross-Domain Few-Shot Object Detection via Enhanced Open-Set Object Detector\\
\noindent\textit{\textbf{Members: }} \\
Yuqian Fu$^1$ (\href{mailto:yuqian.fu@insait.ai}{yuqian.fu@insait.ai}),\\
Yu Wang$^2$, \\
Yixuan Pan$^3$, \\
Xingyu Qiu$^2$, \\
$^1$ INSAIT \\
$^2$ Fudan University  \\
$^3$ Southeast University\\



==> teams/team00_Example/main.tex <==
\subsection{Example}
\subsubsection{Proposed Method}
We propsose a novel CD-ViTO method for the CD-FSOD, under the close-set setting, which only takes COCO as source data and transfer the model to novel target. 
As in Fig.~\ref{fig:framework}, we build our CD-ViTO upon one open-set detector (DE-ViT) and finetune our method using few labeled instances of target domain. Modules in blue are inherited from DE-ViT while modules in orange are proposed by us. New improvements include learnable instance features, instance reweighting, domain prompter, and finetuning;  

\begin{figure}[h]
\vspace{-0.1in}
\centering	{\includegraphics[width=1.\linewidth]{teams/team00_Example/framework.jpg}}
\vspace{-0.1in}
\caption{(a) Overall framework of CD-ViTO. \label{fig:framework} 
}
\vspace{-0.15in}
\end{figure}

Specifically, given $S$ and $q$ as input, we perform the same steps as DE-ViT to obtain instance features $F_{ins} =\{F_{ins}^{ob}, F_{ins}^{bg}\}$, region proposals $R_{q}$, visual features $F_{q}$, and ROI features $F_{q_{roi}}$.
But different from directly averaging $F_{ins}^{ob}$ to obtain class prototypes $F_{pro}^{ob}$ for objects, we first utilize our $M_{LIF}$ to make the precalculated $F_{ins}$ learnable and adapt them by performing the disentangled detection tasks i.e., the localization task supervised by $\mathcal{L}_{loc}$ and the classification task supervised by $\mathcal{L}_{cls}$. 
we apply our $M_{LR}$ to reweight the weights of object instances features $F_{ins}^{ob}$. Generally, $M_{LR}$ is expected to assign higher values to the high-quality instances with slight IB. In this way, the high-quality instances could contribute more to its class prototype. The $M_{LR}$ is inserted after the $M_{LIF}$ and is optimized use the same $\mathcal{L}_{loc}$, $\mathcal{L}_{cls}$.
In addition, to make the model more robust to the changing styles, our proposed $M_{DP}$ is applied to synthesize several virtual "domains" $F_{domain}$. The goal of the $M_{DP}$ is to introduce such domain perturbations and force our features to be consistent with different domains. To ensure the diversity of the introduced domains and constrain the domains would not affect the semantics of features, an extra loss $\mathcal{L}_{dp}$ is introduced. The $M_{DP}$ is build upon the object prototypes $F_{pro}^{ob}$ and the $\mathcal{L}_{dp}$ works with the $\mathcal{L}_{loc}$ and $\mathcal{L}_{cls}$ together.

As for finetuning, we finetune the top two modules i.e., the $M_{DET}$ and $M_{CLS}$. 
via the object function $\mathcal{L}$ as:
\begin{equation}\label{eq:loss}
\mathcal{L}  = \mathcal{L}_{loc} + \mathcal{L}_{cls} + \mathcal{L}_{dp}.
\end{equation}


\noindent \textbf{Learnable Instance Features $M_{LIF}$.}
% The implementation of our learnable instance features $M_{LIF}$ is quiet easy and efficient. 
Given the precalculated instance features $F_{ins} \in \mathcal{R}^{(N \times K + N_{bg}) \times D}$, where $N$, $K$, $N_{bg}$, $D$ represents the number of object classes, the number of shots, the number of background instances, and the dimension of visual features, $M_{LIF}$ defines a new learnable matrix $F_{ins}^{lea}$ with the same size of $F_{ins}$ and use the $F_{ins}$ for initialization. 

\noindent \textbf{Instance Reweighting Module $M_{IR}$.}
Our $M_{IR}$ is proposed to reweight the instances enabling high-quality object instances e.g., objects with slight IB contribute more to the class prototype. 
% The architecture of $M_{IR}$ is shown in Fig.~\ref{fig:framework}(b). 
Given the learnable instance features $F_{ins}^{lea}$ from $M_{LIF}$, we first obtain the object instance features from  $F_{ins}^{lea}$ and denote it as $F_{ins}^{0} \in \mathcal{R}^{N \times K \times D}$. Our $M_{IR}$ has two paths connected in a residual way. 
More specifically, the lower path feeds the $F_{ins}^{0}$ into an MLP module to get the weighted score which is further used to perform the weighted sum on the initial $F_{ins}^{0}$ resulting in the deformed prototypes $F_{ins}^{att} \in \mathcal{R}^{N \times D}$. The upper path performs the average operation on $F_{ins}^{0}$ getting $F_{ins}^{avg} \in \mathcal{R}^{N \times D}$. The final object prototypes $F_{pro}^{ob}$ are represented as $\alpha fc(F_{ins}^{att}) + (1-\alpha)F_{ins}^{avg}$, where the $fc(\cdot)$ denotes a fully connected layer and $\alpha$ is a hyperparameter.  



\noindent \textbf{Domain Prompter $M_{DP}$.}

Given $F_{domain}$ and $F_{pro}^{ob}$, we first propose the domain diversity loss $\mathcal{L}_{domain}$ to force the different domains e.g., $f^{d_{i}}$ and $f^{d_j}$ to be far from each other. Secondly, for a prototype $f_{p_{i}}$ in $F_{pro}^{ob}$, we randomly perturbs it with two various domains $f^{d_{k}}$ and $f^{d_{m}}$ sampled from $F_{domain}$ forming two perturbed prototypes $f_{p_{i}}^{d_{k}}, f_{p_{i}}^{d_{m}}$. The perturbation is done by adding the features e.g., $f_{p_{i}}^{d_{k}} = f_{p_{i}} +f^{d_{k}}$. 
The domain $f^{d_{m}}$ is also added to other object prototypes forming $f_{p_{j}}^{d_{m}}$, where $j = 1, \ldots, N$. 
We constrain that $f_{p_{i}}^{d_{k}}$ and $f_{p_{i}}^{d_{m}}$ should be close to each other while being distant from perturbed prototypes generated from different class prototypes.
This constitutes our prototype consistency loss $\mathcal{L}_{proto}$.  Both the $\mathcal{L}_{domain}$ and $\mathcal{L}_{proto}$ are implemented by the InfoNCE loss.

\subsubsection{Training Details}
we adopt the "pretrain, finetune, and test" pipeline. 
In the case of our CD-ViTO, the base DE-ViT model pretrained on COCO is taken, then the $M_{DET}$, $M_{CLS}$, $M_{LIF}$, $M_{IR}$, and $M_{DP}$ are tuned on novel support images $S$ using the loss as in Eq.~\ref{eq:loss}.
The hyperparameter $N_{bg}$, $\alpha$ ratio of instance reweighting module, $\tau$ temperature for $\mathcal{L}_{proto}$, $\tau$ temperature for $\mathcal{L}_{domain}$  are set as 530, 0.7, 2, 0.1 for all the target datasets. While the value $N_{dom}$ means the number of virtual domains depending on the number of target classes $N$, specifically, we have $N_{dom} = 2*N$.  The hyperparameter Top-K ($K$) in DE-ViT is set as 5. For datasets with number of classes $N$ less than 5, we have $K=N$. We tune the trainable parameters on 1-shot around 80 epochs, and on 5/10-shot around 40 epochs. The SGD with the learning rate as 0.002 is used as the optimizer. Experiments are performed on four RTX3090 GPUs.



==> teams/team02_VIS/affiliation.tex <==
\subsection*{VIS}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team02_VIS/main.tex <==
\subsection{VIS}

==> teams/team04_RLG/affiliation.tex <==
\subsection*{RLG}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team04_RLG/main.tex <==
\subsection{RLG}

==> teams/team09_TechnoTitans/affiliation.tex <==
\subsection*{TechnoTitans}
\noindent\textit{\textbf{Title: }} Title of your Paper or Methods\\
\noindent\textit{\textbf{Members: }} \\
Team member 1$^1$ (\href{mailto:yourEmail@xxx.xxx}{yourEmail@xxx.xxx}),\\
Team member 2$^2$, \\
Team member 3$^3$, \\
\noindent\textit{\textbf{Affiliations: }} \\ 
$^1$ Affiliation 1 \\
$^2$ Affiliation 2 \\
$^3$ Affiliation 3 \\



==> teams/team09_TechnoTitans/main.tex <==
\subsection{TechnoTitans}
